PICCOLO: Point Cloud-Centric Omnidirectional Localization

We present PICCOLO, a simple and efficient algorithm for omnidirectional localization. Given a colored point cloud and a 360 panorama image of a scene, our objective is to recover the camera pose at which the panorama image is taken. Our pipeline works in an off-the-shelf manner with a single image given as a query and does not require any training of neural networks or collecting ground-truth poses of images. Instead, we match each point cloud color to the holistic view of the panorama image with gradient-descent optimization to find the camera pose. Our loss function, called sampling loss, is point cloud-centric, evaluated at the projected location of every point in the point cloud. In contrast, conventional photometric loss is image-centric, comparing colors at each pixel location. With a simple change in the compared entities, sampling loss effectively overcomes the severe visual distortion of omnidirectional images, and enjoys the global context of the 360 view to handle challenging scenarios for visual localization. PICCOLO outperforms existing omnidirectional localization algorithms in both accuracy and stability when evaluated in various environments. Code is available at \url{https://github.com/82magnolia/panoramic-localization/}.

==> assets/images/loss_functions_figure.tex <==
\begin{figure}[t]
\centering
    \begin{subfigure}{.475\linewidth}
    \includegraphics[width=\linewidth]{assets/images/square.png}
    \caption{Scene Coordinate Loss}
    \end{subfigure}
    \begin{subfigure}{.475\linewidth}
    \includegraphics[width=\linewidth]{assets/images/square.png}
    \caption{Reprojection Loss}
    \end{subfigure}
    \newline
    \begin{subfigure}{.475\linewidth}
    \includegraphics[width=\linewidth]{assets/images/square.png}
    \caption{Synthesized Image Loss}
    \end{subfigure}
    \begin{subfigure}{.475\linewidth}
    \includegraphics[width=\linewidth]{assets/images/square.png}
    \caption{Sampling Loss}
    \end{subfigure}
    \caption{Visual illustration of three loss functions along with sampling loss utilized in OmniLoc.}
\label{loss_functions}
\end{figure}

==> assets/images/loss_surface_black.tex <==
\begin{figure*}[t]
\centering
    \includegraphics[width=0.95\textwidth]{assets/images/loss_surface/loss_surfaces_black.png}
\vspace{-0.5em}
\label{loss_surfaces}
\caption{loss surfaces, initial points, ...}
\vspace{-0.5em}
\end{figure*}

==> assets/images/sift_hard.tex <==
\if 0
\begin{figure}[]
\makebox[\columnwidth][c]{
    \includegraphics[width=0.45\linewidth]{assets/images/teaser/compare_gosma/area_2_auditorium_1_2bdad37095ce4485a964cfe4ad8640d9_overlayed_new.jpg}
    \includegraphics[width=0.45\linewidth]{assets/images/teaser/compare_gosma/camera_2bdad37095ce4485a964cfe4ad8640d9_auditorium_1_frame_equirectangular_domain_rgb_new.jpg}
}
\makebox[\columnwidth][c]{
    \includegraphics[width=0.45\linewidth]{assets/images/teaser/compare_gosma/area_6_hallway_2_04a585f344fb462fba9e271912f9feb3_overlayed_new.jpg}
    \includegraphics[width=0.45\linewidth]{assets/images/teaser/compare_gosma/camera_04a585f344fb462fba9e271912f9feb3_hallway_2_frame_equirectangular_domain_rgb_new.jpg}
}

\makebox[\columnwidth][c]{
    \includegraphics[width=0.45\linewidth]{assets/images/teaser/compare_gosma/area_5_office_22_7a42df17b40c4c15bfd6301823b6a476_overlayed_new.jpg}
    \includegraphics[width=0.45\linewidth]{assets/images/teaser/compare_gosma/camera_7a42df17b40c4c15bfd6301823b6a476_office_22_frame_equirectangular_domain_rgb_new.jpg}
}

\makebox[\columnwidth][c]{
    \includegraphics[width=0.45\linewidth]{assets/images/teaser/compare_gosma/area_3_lounge_1_4a7bfe0577f74a1a891683cf5b435f93_overlayed_new.jpg}
    \includegraphics[width=0.45\linewidth]{assets/images/teaser/compare_gosma/camera_4a7bfe0577f74a1a891683cf5b435f93_lounge_1_frame_equirectangular_domain_rgb_new.jpg}
}

\makebox[\columnwidth][c]{
    \makebox[0.45\columnwidth][c]{
        \textit{PICCOLO}
    }
    \makebox[0.45\columnwidth][c]{
        \textit{GOSMA}
    }
}
\caption{Sample data from Stanford2D-3D-S~\cite{stanford2d3d}, MPO~\cite{fukuoka}, and OmniScenes, which lack visual features and exhibit repetitive structure.}
\label{sift_hard_why}
\end{figure}
\fi

\begin{figure}[]
\centering
    \begin{subfigure}[t]{1.0\linewidth}
    \makebox[\columnwidth][c]{
    \includegraphics[width=0.48\linewidth]{assets/images/sift_evidence/hallway_1.jpg}
    \includegraphics[width=0.48\linewidth]{assets/images/sift_evidence/hallway_2.jpg}
    }
    \caption{Stanford2D-3D-S Hallways}
    \label{stanford_hallway}
    \end{subfigure}

    \begin{subfigure}[t]{1.0\linewidth}
    \makebox[\columnwidth][c]{
    \includegraphics[width=0.48\linewidth]{assets/images/sift_evidence/bathroom_1.jpg}
    \includegraphics[width=0.48\linewidth]{assets/images/sift_evidence/bathroom_2.jpg}
    }
    \caption{Stanford2D-3D-S Bathrooms}
    \label{stanford_bathroom}
    \end{subfigure}

    \begin{subfigure}[t]{1.0\linewidth}
    \makebox[\columnwidth][c]{
    \includegraphics[width=0.48\linewidth]{assets/images/sift_evidence/auditorium_1.jpg}
    \includegraphics[width=0.48\linewidth]{assets/images/sift_evidence/auditorium_2.jpg}
    }
    \caption{Stanford2D-3D-S Auditoriums}
    \label{stanford_auditorium}
    \end{subfigure}

    \begin{subfigure}[t]{1.0\linewidth}
    \makebox[\columnwidth][c]{
    \includegraphics[width=0.48\linewidth]{assets/images/sift_evidence/semantic_1.jpg}
    \includegraphics[width=0.48\linewidth]{assets/images/sift_evidence/semantic_2.jpg}
    }
    \caption{Stanford2D-3D-S Semantic Input}
    \label{stanford_semantic}
    \end{subfigure}

    \begin{subfigure}[t]{1.0\linewidth}
    \makebox[\columnwidth][c]{
    \includegraphics[width=0.48\linewidth]{assets/images/sift_evidence/forrest_1.jpg}
    \includegraphics[width=0.48\linewidth]{assets/images/sift_evidence/coast_1.jpg}
    }
    \caption{MPO}
    \label{mpo_supp_sift}
    \end{subfigure}

\caption{Sample data from Stanford2D-3D-S~\cite{stanford2d3d} and MPO~\cite{fukuoka} which lack visual features and exhibit repetitive structure.}
\label{sift_hard_why}
\end{figure}

==> assets/images/stanford_roc_area.tex <==
\begin{figure*}
\centering
    \begin{subfigure}{.33\textwidth}
    \includegraphics[width=\linewidth]{assets/images/ROC/ROC_area_1.pdf}
    \caption{Area 1}
    \end{subfigure}
    \begin{subfigure}{.33\textwidth}
    \includegraphics[width=\linewidth]{assets/images/ROC/ROC_area_2.pdf}
    \caption{Area 2}
    \end{subfigure}
    \begin{subfigure}{.33\textwidth}
    \includegraphics[width=\linewidth]{assets/images/ROC/ROC_area_3.pdf}
    \caption{Area 3}
    \end{subfigure}
    \newline
    \begin{subfigure}{.33\textwidth}
    \includegraphics[width=\linewidth]{assets/images/ROC/ROC_area_4.pdf}
    \caption{Area 4}
    \end{subfigure}
    \begin{subfigure}{.33\textwidth}
    \includegraphics[width=\linewidth]{assets/images/ROC/ROC_area_5.pdf}
    \caption{Area 5}
    \end{subfigure}
    \begin{subfigure}{.33\textwidth}
    \includegraphics[width=\linewidth]{assets/images/ROC/ROC_area_6.pdf}
    \caption{Area 6}
    \end{subfigure}
    \caption{ROC}
\label{stanford_roc_all}
\end{figure*}

==> assets/images/sup_fukuoka.tex <==
\begin{figure*}[h]
\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Coast.1_Scan_002_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Coast.1_Scan_003_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Coast.2_Scan_003_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Coast.3_Scan_009_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Coast.1_Scan_002_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Coast.1_Scan_003_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Coast.2_Scan_003_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Coast.3_Scan_009_proj.jpg}
    }
    \caption{Coast}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Forest.1_Scan_003_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Forest.2_Scan_001_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Forest.3_Scan_001_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Forest.4_Scan_015_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Forest.1_Scan_003_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Forest.2_Scan_001_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Forest.3_Scan_001_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Forest.4_Scan_015_proj.jpg}
    }
    \caption{Forest}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/ParkingIn.1_Scan_002_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/ParkingIn.1_Scan_012_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/ParkingIn.2_Scan_003_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/ParkingIn.7_Scan_005_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/ParkingIn.1_Scan_002_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/ParkingIn.1_Scan_012_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/ParkingIn.2_Scan_003_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/ParkingIn.7_Scan_005_proj.jpg}
    }
    \caption{ParkingIn}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/ParkingOut.2_Scan_011_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/ParkingOut.5_Scan_009_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/ParkingOut.6_Scan_002_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/ParkingOut.7_Scan_014_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/ParkingOut.2_Scan_011_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/ParkingOut.5_Scan_009_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/ParkingOut.6_Scan_002_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/ParkingOut.7_Scan_014_proj.jpg}
    }
    \caption{ParkingOut}
\end{subfigure}

\if 0
\begin{subfigure}[t]{0.5\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.48\linewidth]{assets/images/teaser_new/sup_mpo/ParkingIn.1_Scan_002_gt.jpg}
    \includegraphics[width=0.48\linewidth]{assets/images/teaser_new/sup_mpo/ParkingIn.1_Scan_012_gt.jpg}
    }
\makebox[\textwidth][c]{
    \includegraphics[width=0.48\linewidth]{assets/images/teaser_new/sup_mpo/ParkingIn.1_Scan_002_proj.jpg}
    \includegraphics[width=0.48\linewidth]{assets/images/teaser_new/sup_mpo/ParkingIn.1_Scan_012_proj.jpg}
    }
    \caption{ParkingIn}
\end{subfigure}
\begin{subfigure}[t]{0.5\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.48\linewidth]{assets/images/teaser_new/sup_mpo/ParkingOut.2_Scan_011_gt.jpg}
    \includegraphics[width=0.48\linewidth]{assets/images/teaser_new/sup_mpo/ParkingOut.5_Scan_009_gt.jpg}
    }
\makebox[\textwidth][c]{
    \includegraphics[width=0.48\linewidth]{assets/images/teaser_new/sup_mpo/ParkingOut.2_Scan_011_proj.jpg}
    \includegraphics[width=0.48\linewidth]{assets/images/teaser_new/sup_mpo/ParkingOut.5_Scan_009_proj.jpg}
    }
    \caption{ParkingOut}
\end{subfigure}
\fi

\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Residential.1_Scan_002_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Residential.1_Scan_011_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Residential.2_Scan_006_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Residential.4_Scan_004_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Residential.1_Scan_002_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Residential.1_Scan_011_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Residential.2_Scan_006_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Residential.4_Scan_004_proj.jpg}
    }
    \caption{Residential}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Urban.1_Scan_002_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Urban.1_Scan_009_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Urban.3_Scan_001_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Urban.6_Scan_003_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Urban.1_Scan_002_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Urban.1_Scan_009_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Urban.3_Scan_001_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_mpo/Urban.6_Scan_003_proj.jpg}
    }
    \caption{Urban}
\end{subfigure}

\vspace{-0.7em}
\caption{Qualitative results of PICCOLO. We display the input query image (top) and the projected point cloud under the estimated camera pose (bottom).}
\label{mpo_supp}
\vspace{-0.7em}
\end{figure*}

==> assets/images/sup_nicta.tex <==
\begin{figure*}[h!]

\makebox[\textwidth][c]{
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene2_frame260_gt.jpg}
    \hspace{0.01\linewidth}
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene2_frame260_proj.jpg}
    \hspace{0.01\linewidth}
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene2_frame260_overlay.jpg}
}

\makebox[\textwidth][c]{
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene3_frame482_gt.jpg}
    \hspace{0.01\linewidth}
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene3_frame482_proj.jpg}
    \hspace{0.01\linewidth}
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene3_frame482_overlay.jpg}
}

\makebox[\textwidth][c]{
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene4_frame750_gt.jpg}
    \hspace{0.01\linewidth}
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene4_frame750_proj.jpg}
    \hspace{0.01\linewidth}
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene4_frame750_overlay.jpg}
}

\makebox[\textwidth][c]{
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene5_frame809_gt.jpg}
    \hspace{0.01\linewidth}
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene5_frame809_proj.jpg}
    \hspace{0.01\linewidth}
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene5_frame809_overlay.jpg}
}

\makebox[\textwidth][c]{
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene7_frame2455_gt.jpg}
    \hspace{0.01\linewidth}
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene7_frame2455_proj.jpg}
    \hspace{0.01\linewidth}
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene7_frame2455_overlay.jpg}
}

\makebox[\textwidth][c]{
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene8_frame3195_gt.jpg}
    \hspace{0.01\linewidth}
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene8_frame3195_proj.jpg}
    \hspace{0.01\linewidth}
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene8_frame3195_overlay.jpg}
}

\makebox[\textwidth][c]{
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene9_frame3380_gt.jpg}
    \hspace{0.01\linewidth}
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene9_frame3380_proj.jpg}
    \hspace{0.01\linewidth}
    \includegraphics[width=0.28\linewidth]{assets/images/teaser/sup_nicta/scene9_frame3380_overlay.jpg}
}

\makebox[\textwidth][c]{
    \makebox[0.28\textwidth][c]{
        \textit{Query Image}
    }
    \hspace{0.01\linewidth}
    \makebox[0.28\textwidth][c]{
        \textit{Projected Point Cloud}
    }
    \hspace{0.01\linewidth}
    \makebox[0.28\textwidth][c]{
        \textit{Overlaid Point Cloud}
    }
}
\caption{Qualitative results of OmniLoc.}
\label{sup_nicta}
\vspace{-1.0em}
\end{figure*}

==> assets/images/sup_omni_scene1_hand.tex <==
\begin{figure*}[h]
\begin{center}
\begin{subfigure}[t]{0.49\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_hand/sup_omni_scene1_hand_wed_1_query.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_hand/sup_omni_scene1_hand_wed_2_query.jpg}
    }
\makebox[\textwidth][c]{
     \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_hand/sup_omni_scene1_hand_wed_1_proj.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_hand/sup_omni_scene1_hand_wed_2_proj.jpg}
    }
    \caption{Wedding Hall}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_hand/sup_omni_scene1_hand_trad_1_query.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_hand/sup_omni_scene1_hand_trad_2_query.jpg}
    }
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_hand/sup_omni_scene1_hand_trad_1_proj.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_hand/sup_omni_scene1_hand_trad_2_proj.jpg}
    }
    \caption{Traditional Room}
\end{subfigure}
\end{center}
\begin{center}
\vspace{-1em}
\begin{subfigure}[t]{0.49\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_hand/sup_omni_scene1_hand_room1_1_query.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_hand/sup_omni_scene1_hand_room1_2_query.jpg}
    }
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_hand/sup_omni_scene1_hand_room1_1_proj.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_hand/sup_omni_scene1_hand_room1_2_proj.jpg}
    }
    \caption{Hotel Room 1}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_hand/sup_omni_scene1_hand_room2_1_query.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_hand/sup_omni_scene1_hand_room2_2_query.jpg}
    }
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_hand/sup_omni_scene1_hand_room2_1_proj.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_hand/sup_omni_scene1_hand_room2_2_proj.jpg}
    }
    \caption{Hotel Room 2}
\end{subfigure}
\end{center}
\vspace{-0.5em}
\setlength\abovecaptionskip{-5pt}
\caption{Qualitative results of PICCOLO. We display the input query image (top) and the projected point cloud under the estimated camera pose (bottom).}
\label{sup_omni_scene1_hand}
\vspace{-0.5em}
\end{figure*}

==> assets/images/sup_omni_scene1_robot.tex <==
\begin{figure*}[b]
\begin{center}
\begin{subfigure}[t]{0.49\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_robot/sup_omni_scene1_robot_wed_1_query.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_robot/sup_omni_scene1_robot_wed_2_query.jpg}
    }
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_robot/sup_omni_scene1_robot_wed_1_proj.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_robot/sup_omni_scene1_robot_wed_2_proj.jpg}
    }
    \caption{Wedding Hall}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_robot/sup_omni_scene1_robot_trad_1_query.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_robot/sup_omni_scene1_robot_trad_2_query.jpg}
    }
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_robot/sup_omni_scene1_robot_trad_1_proj.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_robot/sup_omni_scene1_robot_trad_2_proj.jpg}
    }
    \caption{Traditional Room}
\end{subfigure}
\end{center}
\begin{center}
\vspace{-1em}
\begin{subfigure}[t]{0.49\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_robot/sup_omni_scene1_robot_room1_1_query.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_robot/sup_omni_scene1_robot_room1_2_query.jpg}
    }
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_robot/sup_omni_scene1_robot_room1_1_proj.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_robot/sup_omni_scene1_robot_room1_2_proj.jpg}
    }
    \caption{Hotel Room 1}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_robot/sup_omni_scene1_robot_room2_1_query.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_robot/sup_omni_scene1_robot_room2_2_query.jpg}
    }
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_robot/sup_omni_scene1_robot_room2_1_proj.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene1_robot/sup_omni_scene1_robot_room2_2_proj.jpg}
    }
    \caption{Hotel Room 2}
\end{subfigure}
\end{center}
\vspace{-0.5em}
\setlength\abovecaptionskip{-5pt}
\caption{Qualitative results of PICCOLO. We display the input query image (top) and the projected point cloud under the estimated camera pose (bottom).}
\label{sup_omni_scene1_robot}
\vspace{-0.5em}


\if 0
\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_1_camera_7c870c23c35c4480b05a45083f704ff0_hallway_8_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_3_camera_87a1bc34ffb4408ba077119216ed763e_hallway_2_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_4b6982edad14499bbc5cb606f85242f3_hallway_10_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_1e80852fb4b2410db6372e0b03519f4a_hallway_5_frame_equirectangular_domain_rgb_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_1_camera_7c870c23c35c4480b05a45083f704ff0_hallway_8_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_3_camera_87a1bc34ffb4408ba077119216ed763e_hallway_2_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_4b6982edad14499bbc5cb606f85242f3_hallway_10_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_1e80852fb4b2410db6372e0b03519f4a_hallway_5_frame_equirectangular_domain_rgb_proj.jpg}
    }
    \caption{Hallway}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_1_camera_7c870c23c35c4480b05a45083f704ff0_hallway_8_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_3_camera_87a1bc34ffb4408ba077119216ed763e_hallway_2_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_4b6982edad14499bbc5cb606f85242f3_hallway_10_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_1e80852fb4b2410db6372e0b03519f4a_hallway_5_frame_equirectangular_domain_rgb_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_1_camera_7c870c23c35c4480b05a45083f704ff0_hallway_8_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_3_camera_87a1bc34ffb4408ba077119216ed763e_hallway_2_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_4b6982edad14499bbc5cb606f85242f3_hallway_10_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_1e80852fb4b2410db6372e0b03519f4a_hallway_5_frame_equirectangular_domain_rgb_proj.jpg}
    }
    \caption{Hallway}
\end{subfigure}
\vspace{-0.5em}
\setlength\abovecaptionskip{-5pt}
\caption{Qualitative results of PICCOLO. We display the input query image (top) and the projected point cloud under the estimated camera pose (bottom).}
\label{sup_omni_scene1_robot}
\vspace{-0.5em}
\fi
\end{figure*}

==> assets/images/sup_omni_scene2_hand.tex <==
\begin{figure*}[h]
\begin{center}
\begin{subfigure}[t]{0.49\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_hand/sup_omni_scene2_hand_wed_1_query.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_hand/sup_omni_scene2_hand_wed_2_query.jpg}
    }
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_hand/sup_omni_scene2_hand_wed_1_proj.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_hand/sup_omni_scene2_hand_wed_2_proj.jpg}
    }
    \caption{Wedding Hall}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_hand/sup_omni_scene2_hand_trad_1_query.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_hand/sup_omni_scene2_hand_trad_2_query.jpg}
    }
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_hand/sup_omni_scene2_hand_trad_1_proj.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_hand/sup_omni_scene2_hand_trad_2_proj.jpg}
    }
    \caption{Traditional Room}
\end{subfigure}
\end{center}
\begin{center}
\vspace{-1em}
\begin{subfigure}[t]{0.49\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_hand/sup_omni_scene2_hand_room1_1_query.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_hand/sup_omni_scene2_hand_room1_2_query.jpg}
    }
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_hand/sup_omni_scene2_hand_room1_1_proj.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_hand/sup_omni_scene2_hand_room1_2_proj.jpg}
    }
    \caption{Hotel Room 1}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_hand/sup_omni_scene2_hand_room2_1_query.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_hand/sup_omni_scene2_hand_room2_2_query.jpg}
    }
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_hand/sup_omni_scene2_hand_room2_1_proj.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_hand/sup_omni_scene2_hand_room2_2_proj.jpg}
    }
    \caption{Hotel Room 2}
\end{subfigure}
\end{center}
\vspace{-0.5em}
\setlength\abovecaptionskip{-5pt}
\caption{Qualitative results of PICCOLO. We display the input query image (top) and the projected point cloud under the estimated camera pose (bottom).}
\label{sup_omni_scene2_hand}
\vspace{-0.5em}


\if 0
\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_1_camera_7c870c23c35c4480b05a45083f704ff0_hallway_8_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_3_camera_87a1bc34ffb4408ba077119216ed763e_hallway_2_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_4b6982edad14499bbc5cb606f85242f3_hallway_10_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_1e80852fb4b2410db6372e0b03519f4a_hallway_5_frame_equirectangular_domain_rgb_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_1_camera_7c870c23c35c4480b05a45083f704ff0_hallway_8_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_3_camera_87a1bc34ffb4408ba077119216ed763e_hallway_2_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_4b6982edad14499bbc5cb606f85242f3_hallway_10_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_1e80852fb4b2410db6372e0b03519f4a_hallway_5_frame_equirectangular_domain_rgb_proj.jpg}
    }
    \caption{Hallway}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_1_camera_7c870c23c35c4480b05a45083f704ff0_hallway_8_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_3_camera_87a1bc34ffb4408ba077119216ed763e_hallway_2_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_4b6982edad14499bbc5cb606f85242f3_hallway_10_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_1e80852fb4b2410db6372e0b03519f4a_hallway_5_frame_equirectangular_domain_rgb_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_1_camera_7c870c23c35c4480b05a45083f704ff0_hallway_8_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_3_camera_87a1bc34ffb4408ba077119216ed763e_hallway_2_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_4b6982edad14499bbc5cb606f85242f3_hallway_10_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_1e80852fb4b2410db6372e0b03519f4a_hallway_5_frame_equirectangular_domain_rgb_proj.jpg}
    }
    \caption{Hallway}
\end{subfigure}
\vspace{-0.5em}
\setlength\abovecaptionskip{-5pt}
\caption{Qualitative results of PICCOLO. We display the input query image (top) and the projected point cloud under the estimated camera pose (bottom).}
\label{sup_omni_scene1_robot}
\vspace{-0.5em}
\fi
\end{figure*}

==> assets/images/sup_omni_scene2_robot.tex <==
\begin{figure*}[b]
\begin{center}
\begin{subfigure}[t]{0.49\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_robot/sup_omni_scene2_robot_wed_1_query.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_robot/sup_omni_scene2_robot_wed_2_query.jpg}
    }
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_robot/sup_omni_scene2_robot_wed_1_proj.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_robot/sup_omni_scene2_robot_wed_2_proj.jpg}
    }
    \caption{Wedding Hall}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_robot/sup_omni_scene2_robot_trad_1_query.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_robot/sup_omni_scene2_robot_trad_2_query.jpg}
    }
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_robot/sup_omni_scene2_robot_trad_1_proj.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_robot/sup_omni_scene2_robot_trad_2_proj.jpg}
    }
    \caption{Traditional Room}
\end{subfigure}
\end{center}
\begin{center}
\vspace{-1em}
\begin{subfigure}[t]{0.49\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_robot/sup_omni_scene2_robot_room1_1_query.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_robot/sup_omni_scene2_robot_room1_2_query.jpg}
    }
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_robot/sup_omni_scene2_robot_room1_1_proj.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_robot/sup_omni_scene2_robot_room1_2_proj.jpg}
    }
    \caption{Hotel Room 1}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_robot/sup_omni_scene2_robot_room2_1_query.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_robot/sup_omni_scene2_robot_room2_2_query.jpg}
    }
\makebox[\textwidth][c]{
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_robot/sup_omni_scene2_robot_room2_1_proj.jpg}
    \includegraphics[width=0.47\linewidth]{assets/images/teaser_new/sup_omni_scene2_robot/sup_omni_scene2_robot_room2_2_proj.jpg}
    }
    \caption{Hotel Room 2}
\end{subfigure}
\end{center}
\vspace{-0.5em}
\setlength\abovecaptionskip{-5pt}
\caption{Qualitative results of PICCOLO. We display the input query image (top) and the projected point cloud under the estimated camera pose (bottom).}
\label{sup_omni_scene2_robot}
\vspace{-0.5em}


\if 0
\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_1_camera_7c870c23c35c4480b05a45083f704ff0_hallway_8_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_3_camera_87a1bc34ffb4408ba077119216ed763e_hallway_2_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_4b6982edad14499bbc5cb606f85242f3_hallway_10_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_1e80852fb4b2410db6372e0b03519f4a_hallway_5_frame_equirectangular_domain_rgb_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_1_camera_7c870c23c35c4480b05a45083f704ff0_hallway_8_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_3_camera_87a1bc34ffb4408ba077119216ed763e_hallway_2_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_4b6982edad14499bbc5cb606f85242f3_hallway_10_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_1e80852fb4b2410db6372e0b03519f4a_hallway_5_frame_equirectangular_domain_rgb_proj.jpg}
    }
    \caption{Hallway}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_1_camera_7c870c23c35c4480b05a45083f704ff0_hallway_8_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_3_camera_87a1bc34ffb4408ba077119216ed763e_hallway_2_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_4b6982edad14499bbc5cb606f85242f3_hallway_10_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_1e80852fb4b2410db6372e0b03519f4a_hallway_5_frame_equirectangular_domain_rgb_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_1_camera_7c870c23c35c4480b05a45083f704ff0_hallway_8_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_3_camera_87a1bc34ffb4408ba077119216ed763e_hallway_2_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_4b6982edad14499bbc5cb606f85242f3_hallway_10_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.23\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_1e80852fb4b2410db6372e0b03519f4a_hallway_5_frame_equirectangular_domain_rgb_proj.jpg}
    }
    \caption{Hallway}
\end{subfigure}
\vspace{-0.5em}
\setlength\abovecaptionskip{-5pt}
\caption{Qualitative results of PICCOLO. We display the input query image (top) and the projected point cloud under the estimated camera pose (bottom).}
\label{sup_omni_scene1_robot}
\vspace{-0.5em}
\fi
\end{figure*}

==> assets/images/sup_semantic.tex <==
\begin{figure*}[h]
\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_1_camera_4ff66baf78ae47e0bbd6443312ba648e_office_30_frame_equirectangular_domain_semantic_pretty_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_3_camera_66dbab011f344dcc9ad643473adff86d_office_7_frame_equirectangular_domain_semantic_pretty_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_5_camera_4f5daf1861574c619838d4b4ed54c5d3_office_15_frame_equirectangular_domain_semantic_pretty_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_6_camera_8f384ebabf6240d49013fc411b501b7e_office_8_frame_equirectangular_domain_semantic_pretty_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_1_camera_4ff66baf78ae47e0bbd6443312ba648e_office_30_frame_equirectangular_domain_semantic_pretty_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_3_camera_66dbab011f344dcc9ad643473adff86d_office_7_frame_equirectangular_domain_semantic_pretty_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_5_camera_4f5daf1861574c619838d4b4ed54c5d3_office_15_frame_equirectangular_domain_semantic_pretty_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_6_camera_8f384ebabf6240d49013fc411b501b7e_office_8_frame_equirectangular_domain_semantic_pretty_proj.jpg}
    }
    \caption{Office}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_2_camera_0e48e05d016544bab840fd9bd6ce5563_auditorium_1_frame_equirectangular_domain_semantic_pretty_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_2_camera_2bdad37095ce4485a964cfe4ad8640d9_auditorium_1_frame_equirectangular_domain_semantic_pretty_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_2_camera_5a4c83dae03248e3b85a7980e0ed5971_auditorium_2_frame_equirectangular_domain_semantic_pretty_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_2_camera_7cf902a1a41742b1a470ae2222d70165_auditorium_2_frame_equirectangular_domain_semantic_pretty_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_2_camera_0e48e05d016544bab840fd9bd6ce5563_auditorium_1_frame_equirectangular_domain_semantic_pretty_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_2_camera_2bdad37095ce4485a964cfe4ad8640d9_auditorium_1_frame_equirectangular_domain_semantic_pretty_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_2_camera_5a4c83dae03248e3b85a7980e0ed5971_auditorium_2_frame_equirectangular_domain_semantic_pretty_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_2_camera_7cf902a1a41742b1a470ae2222d70165_auditorium_2_frame_equirectangular_domain_semantic_pretty_proj.jpg}
    }
    \caption{Auditorium}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_2_camera_1a10d63a687b492fabd1cf737449399f_hallway_8_frame_equirectangular_domain_semantic_pretty_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_3_camera_6cf9b1a7e96d44aeb9a8a147328b6e76_hallway_4_frame_equirectangular_domain_semantic_pretty_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_4_camera_4b6982edad14499bbc5cb606f85242f3_hallway_10_frame_equirectangular_domain_semantic_pretty_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_6_camera_9a1f8e64a0be4ba9ae79d251b39fb9df_hallway_2_frame_equirectangular_domain_semantic_pretty_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_2_camera_1a10d63a687b492fabd1cf737449399f_hallway_8_frame_equirectangular_domain_semantic_pretty_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_3_camera_6cf9b1a7e96d44aeb9a8a147328b6e76_hallway_4_frame_equirectangular_domain_semantic_pretty_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_4_camera_4b6982edad14499bbc5cb606f85242f3_hallway_10_frame_equirectangular_domain_semantic_pretty_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_semantic/area_6_camera_9a1f8e64a0be4ba9ae79d251b39fb9df_hallway_2_frame_equirectangular_domain_semantic_pretty_proj.jpg}
    }
    \caption{Hallway}
\end{subfigure}
\begin{center}
\vspace{-0.7em}
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\linewidth]{assets/images/teaser_new/sup_semantic/area_3_camera_b3ef2004d9fb42ba909f0da483b1a1f9_WC_1_frame_equirectangular_domain_semantic_pretty_gt.jpg}
    \includegraphics[width=\linewidth]{assets/images/teaser_new/sup_semantic/area_3_camera_b3ef2004d9fb42ba909f0da483b1a1f9_WC_1_frame_equirectangular_domain_semantic_pretty_proj.jpg}
    \caption{WC}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\linewidth]{assets/images/teaser_new/sup_semantic/area_3_camera_a024bdaf470f44d6af6813c3b119b38f_lounge_2_frame_equirectangular_domain_semantic_pretty_gt.jpg}
    \includegraphics[width=\linewidth]{assets/images/teaser_new/sup_semantic/area_3_camera_a024bdaf470f44d6af6813c3b119b38f_lounge_2_frame_equirectangular_domain_semantic_pretty_proj.jpg}
    \caption{Lounge}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\linewidth]{assets/images/teaser_new/sup_semantic/area_4_camera_12e1dc346abe4821b36289e7d69d4f6a_lobby_2_frame_equirectangular_domain_semantic_pretty_gt.jpg}
    \includegraphics[width=\linewidth]{assets/images/teaser_new/sup_semantic/area_4_camera_12e1dc346abe4821b36289e7d69d4f6a_lobby_2_frame_equirectangular_domain_semantic_pretty_proj.jpg}
    \caption{Lobby}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\linewidth]{assets/images/teaser_new/sup_semantic/area_6_camera_da79aa8f1ac342909d6661c22544ce6f_openspace_1_frame_equirectangular_domain_semantic_pretty_gt.jpg}
    \includegraphics[width=\linewidth]{assets/images/teaser_new/sup_semantic/area_6_camera_da79aa8f1ac342909d6661c22544ce6f_openspace_1_frame_equirectangular_domain_semantic_pretty_proj.jpg}
    \caption{Openspace}
\end{subfigure}
\end{center}
\vspace{-0.5em}
\caption{Qualitative results of PICCOLO. We display the input query image (top) and the projected point cloud under the estimated camera pose (bottom).}
\label{sup_stanford}
\vspace{-0.5em}
\end{figure*}

==> assets/images/sup_stanford.tex <==
\begin{figure*}[h]
\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_1_office_10_8fd8146acfca462d9fc0c4b80568e006_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_1_office_30_737918e517c940158e75774d9e4be69a_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_0aee52b0e85f48b7a67ed03b48c55fdb_office_21_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_1f3dc743c37e474a80d38ec4937f8e80_office_26_frame_equirectangular_domain_rgb_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_1_office_10_8fd8146acfca462d9fc0c4b80568e006_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_1_office_30_737918e517c940158e75774d9e4be69a_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_0aee52b0e85f48b7a67ed03b48c55fdb_office_21_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_1f3dc743c37e474a80d38ec4937f8e80_office_26_frame_equirectangular_domain_rgb_proj.jpg}
    }
    \caption{Office}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_2_camera_1bbe6544f4214e81b468b35e77d8cf3d_auditorium_2_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_2_camera_2f0eb2cfd91d4caab8ea79a4bbcbd950_auditorium_1_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_2_camera_3f7631689f0e412e9e6d09ae46dce410_auditorium_1_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_2_camera_31ccbba421134b809e529b9971512c14_auditorium_1_frame_equirectangular_domain_rgb_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_2_camera_1bbe6544f4214e81b468b35e77d8cf3d_auditorium_2_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_2_camera_2f0eb2cfd91d4caab8ea79a4bbcbd950_auditorium_1_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_2_camera_3f7631689f0e412e9e6d09ae46dce410_auditorium_1_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_2_camera_31ccbba421134b809e529b9971512c14_auditorium_1_frame_equirectangular_domain_rgb_proj.jpg}
    }
    \caption{Auditorium}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
\makebox[\textwidth][c]{
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_1_camera_7c870c23c35c4480b05a45083f704ff0_hallway_8_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_3_camera_87a1bc34ffb4408ba077119216ed763e_hallway_2_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_4b6982edad14499bbc5cb606f85242f3_hallway_10_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_1e80852fb4b2410db6372e0b03519f4a_hallway_5_frame_equirectangular_domain_rgb_gt.jpg}
    }
% \vspace{1em}
\makebox[\textwidth][c]{
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_1_camera_7c870c23c35c4480b05a45083f704ff0_hallway_8_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_3_camera_87a1bc34ffb4408ba077119216ed763e_hallway_2_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_4b6982edad14499bbc5cb606f85242f3_hallway_10_frame_equirectangular_domain_rgb_proj.jpg}
    \includegraphics[width=0.24\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_1e80852fb4b2410db6372e0b03519f4a_hallway_5_frame_equirectangular_domain_rgb_proj.jpg}
    }
    \caption{Hallway}
\end{subfigure}
\begin{center}
\vspace{-0.7em}
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_d6b7f484132b401d876179d2006b25ff_WC_4_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_d6b7f484132b401d876179d2006b25ff_WC_4_frame_equirectangular_domain_rgb_proj.jpg}
    \caption{WC}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\linewidth]{assets/images/teaser_new/sup_stanford/area_3_camera_80e1f6ae6c4b4e6dac81676ac86cacfb_lounge_1_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=\linewidth]{assets/images/teaser_new/sup_stanford/area_3_camera_80e1f6ae6c4b4e6dac81676ac86cacfb_lounge_1_frame_equirectangular_domain_rgb_proj.jpg}
    \caption{Lounge}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_02c022c6a4eb476b8271a267fb671526_lobby_1_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=\linewidth]{assets/images/teaser_new/sup_stanford/area_4_camera_02c022c6a4eb476b8271a267fb671526_lobby_1_frame_equirectangular_domain_rgb_proj.jpg}
    \caption{Lobby}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_7b3b20f263b740c9a3e41ccdd319d2f8_openspace_1_frame_equirectangular_domain_rgb_gt.jpg}
    \includegraphics[width=\linewidth]{assets/images/teaser_new/sup_stanford/area_6_camera_7b3b20f263b740c9a3e41ccdd319d2f8_openspace_1_frame_equirectangular_domain_rgb_proj.jpg}
    \caption{Openspace}
\end{subfigure}
\end{center}
\vspace{-0.5em}
\caption{Qualitative results of PICCOLO. We display the input query image (top) and the projected point cloud under the estimated camera pose (bottom).}
\label{sup_stanford}
\vspace{-0.5em}
\end{figure*}

==> tables/zhang.tex <==
\begin{table}[]
\centering
\begin{tabular}{c|c|c}
Method       & t-Error(m)     & R-Error($^\circ$)     \\ \hline
PoseNet~\cite{posenet}      & 1.95           & 7.45           \\
SphereNet~\cite{spherenet}    & 2.29           & 26.7           \\
Zhang \etal~\cite{sphere_cnn} & 1.64           & 9.15           \\
OmniLoc & \textbf{0.01} & \textbf{0.22}
\end{tabular}
\caption{Quantitative results of OmniLoc compared against learning-based methods.
Median values of each metric are reported.}
\label{tab:learning}
\end{table}

